Accessible Nonverbal Cues to Support Conversations in VR for Blind and Low Vision People

Social VR has increased in popularity due to its affordances for rich, embodied, and nonverbal communication. However, nonverbal communication remains inaccessible for blind and low vision people in social VR. We designed accessible cues with audio and haptics to represent three nonverbal behaviors: eye contact, head shaking, and head nodding. We evaluated these cues in real-time conversation tasks where 16 blind and low vision participants conversed with two other users in VR. We found that the cues were effective in supporting conversations in VR. Participants had statistically significantly higher scores for accuracy and confidence in detecting attention during conversations with the cues than without. We also found that participants had a range of preferences and uses for the cues, such as learning social norms. We present design implications for handling additional cues in the future, such as the challenges of incorporating AI. Through this work, we take a step towards making interpersonal embodied interactions in VR fully accessible for blind and low vision people.

==> figures/alttexts.tex <==
Figure 1: Two images of the virtual environments that the studies took place in. The left image is a screenshot of a small, white room designed to look like a waiting room. Two orange chairs are placed facing slightly towards each other, and the screenshot is taken as though the viewer is seated in one of the chairs. There is a cabinet against the left wall, a vending machine in the left corner of the room, and a potted plant in the right corner. A TV hangs on the back wall. The right image is a screenshot of a slightly larger white room designed to look like a conference room. There is a long white table with four white chairs placed around it. The screenshot is taken as though the viewer is standing behind one chair. There is a bookshelf against the far wall, a potted plant in the right corner across from the bookshelf, and a large window taking up the right wall.

Figure 2: Two tables depicting the accuracy and confidence scores in a histogram. The left table is titled "Accuracy Scores Histogram (WithoutCues Versus WithCues)". It has three columns: PID, WithoutCues, and WithCues. Under PID, all participant ID numbers are listed from P1 to P16, with each number being assigned a row. Under WithoutCues and WithCues, the participants' accuracy score for each condition is displayed, with colors to indicate if the scores improved WithCues. Almost every row is green, with a few yellow rows scattered in, and one red row. The right table is titled "Confidence Scores Histogram (WithoutCues Versus WithCues)". It is set up with the exact same columns as the previous table. This table has mostly yellow rows, with a few green rows scattered in, and one more red row. In addition, there are four gray rows where participants' scores are written as NA.

Figure 3: A histogram depicting Likert scale responses from participants. The histogram is titled "Usefulness and Distraction Likert Scale Responses Histogram". There are five columns labled 1 through 5, plus two more columns labled "Mean" and "SD". Under the numbers, there are statements listed that participants responded to. Underneath each statement, there are numbers indicating how many participants responded to the statement with the given column number (e.g., if 8 people responded with a score of 5, the "5" column would have the number 8 under the statement). Further, the numbers are color-coded in shades of blue to indicate where the most amount of answers are falling: the deeper blue colors mean more responses, and lighter blues indicate fewer responses. The first statement is "The accessible nonverbal cues were useful to detect if people were paying attention to me or not." The answers are concentrated towards 5, with this column being a very dark blue, and 1-4 being light shades of blue. "Mean" is listed as 3.87 and "SD" is 1.32. The second statement is "The accessible nonverbal cues were distracting." The answers are concentrated towards 2, with this column being a very dark blue, and columns 1, 3, 4, 5 being light shades of blue. "Mean" is listed as 2.53 and "SD" is 1.2.

Figure 4: A histogram depicting Likert scale responses from participants. The histogram is titled "Task Ease Likert Scale Responses Histogram (WithCues Versus WithoutCues)". There are five columns labled 1 through 5, plus two more columns labled "Mean" and "SD". Under the numbers, there are statements listed that participants responded to, with parantheses indicating whether this statement was for the WithCues or WithoutCues condition. Underneath each statement, there are numbers indicating how many participants responded to the statement with the given column number (e.g., if 6 people responded with a score of 5, the "5" column would have the number 6 under the statement). Further, the numbers are color-coded in shades of blue to indicate where the most amount of answers are falling: the deeper blue colors mean more responses, and lighter blues indicate fewer responses. The first statement is "It was easy to determine whether people were paying attention to me or not (WithCues)." The answers are concentrated towards 4 and 5, with these column being very dark blue, and 1-3 being light shades of blue. "Mean" is listed as 4.18 and "SD" is 0.8. The second statement is "It was easy to determine whether people were paying attention to me or not (WithoutCues)." The answers are concentrated towards 4, with this column being a very dark blue, and columns 1, 2, 3, 5 being light shades of blue. "Mean" is listed as 3.62 and "SD" is 0.93.

==> tables/temp.tex <==
\begin{table*}
\centering
\caption{\label{tab: Tasks Table} A table showing the four different task sets, with two counterbalanced attention conditions and one debate topic per each task. }
\begin{tblr}{
  width = \linewidth,
  colspec={Q[30]Q[200]Q[200]Q[200]},
  hlines,
  vlines,
}
\textbf{Set}        
& \textbf{Debate Topic}
& \textbf{Segment 1 Attention\\Condition}     
& \textbf{Segment 2 Attention\\Condition}
\\

A       
& if a hotdog is a sandwich
& Nobody pays attention
& Only Researcher A pays attention

\\

B   
& morning or evening showers are better
& Everyone pays attention
& Only Researcher B pays attention

\\

C       
& if pineapple belongs on pizza
& Only Researcher B pays attention
& Only Researcher A pays attention                                    

\\

D        
& if sandwiches should have crust or no crust
& Everyone pays attention
& Nobody pays attention

\end{tblr}
\end{table*}



